Delving Into Deep Walkers: A Convergence Analysis of Random-Walk-Based Vertex Embeddings

Graph vertex embeddings based on random walks have become increasingly influential in recent years, showing good performance in several tasks as they efficiently transform a graph into a more computationally digestible format while preserving relevant information. However, the theoretical properties of such algorithms, in particular the influence of hyperparameters and of the graph structure on their convergence behaviour, have so far not been well-understood. In this work, we provide a theoretical analysis for random-walks based embeddings techniques. Firstly, we prove that, under some weak assumptions, vertex embeddings derived from random walks do indeed converge both in the single limit of the number of random walks $N \to \infty$ and in the double limit of both $N$ and the length of each random walk $L\to\infty$. Secondly, we derive concentration bounds quantifying the converge rate of the corpora for the single and double limits. Thirdly, we use these results to derive a heuristic for choosing the hyperparameters $N$ and $L$. We validate and illustrate the practical importance of our findings with a range of numerical and visual experiments on several graphs drawn from real-world applications.

==> LaTeX Source/sections/conclusion.tex <==
\vspace{-0.2cm}
\section{Conclusion}\label{sec:conclusion}

We presented a convergence analysis for random-walk-based vertex embeddings. Unlike existing theoretical works, we investigated the convergence of vertex co-occurrences in the generated corpus as the number of random walks $N \to \infty$ for arbitrary random walk lengths $L$ as well as the simultaneous limit $N, L\to \infty$, proving almost sure convergence and quantifying the convergence rates by deriving concentration bounds for the two limits.
We also proved that convergence of vertex co-occurrences does indeed imply convergence of the vertex embeddings themselves, a fact that to our knowledge had not previously received formal theoretical treatment.
Moreover, we provided a heuristic for choosing optimal values for the hyperparameters $N$ and $L$. We supported our theory with a set of experiments using several real-world graphs, and demonstrate the practical implication of our findings.
 

==> LaTeX Source/sections/convergenceestimates.tex <==
\section{Theoretical Analysis}\label{sec:convergence} We can now give our main theoretical results. 
  We first prove convergence of the vertex co-occurrences as $N\to \infty$ and in the joint limit $N, L \to \infty$ in \cref{subsec:convrandomwalks}. We then quantify the rate of these convergences and show how they lead to a heuristic for choosing the hyperparameters $N, L$ in \cref{subsec:convrate}. We finally show in  \cref{subsec:convvertexreps} that, under relatively weak assumptions, convergence of the vertex co-occurrences implies the convergence of the learned vertex representation.
    


\subsection{Convergence of Vertex Co-Occurrences}\label{subsec:convrandomwalks}

    In this section, we derive the limit of the vertex co-occurrences (the frequencies with which a given vertex pair appears in the corpus) as the number of random walks $N$ and then also their length $L$ become infinite.

    \begin{theorem}[Occurrence Vertex Co-Occurrences]\label{thm:relpairoccurrence}
        Let $\mathcal{D}$ be a corpus generated by \Cref{algo:corpusgeneration}. Retaining the notation from that algorithm, the expected relative frequency of occurrence of the pair $(v, c)$ in the corpus is
        %
        \begin{align*}
            \mathbb{E}\bigg[&\frac{m(v, c)}{|\mathcal{D}|}\bigg] = \\
                &\mathbb{E}_{s \sim f_{V_0}} \bigg[\frac{1}{L-T}\sum_{j=0}^{L-T-1} \frac{1}{2T}\sum_{r=1}^T (P^{j})_{sv}(P^r)_{vc} \\
                &\hspace{1cm}+ (P^{j})_{sc}(P^r)_{cv}\bigg].
        \end{align*}
        Furthermore, 
        \begin{equation*}
            \frac{m(v, c)}{|\mathcal{D}|}- \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] \longrightarrow 0\; \textnormal{almost surely as} \; N\rightarrow \infty.
        \end{equation*}
    \end{theorem}

    \begin{IEEEproof}
        A corpus $\mathcal{D}$ generated from $N$ random walks is the union of $N$ independent sub-corpora $\{\mathcal{D}_n\}_{1\leq n\leq N}$, which are each generated from just a single random walk. Thus the expected value of $\frac{m(v, c)}{|\mathcal{D}|}$ is the expected value of $\frac{m_n(v, c)}{|\mathcal{D}_n|}$ (the relative occurrence frequency in sub-corpus $\mathcal{D}_n$), averaged over all $n$. Since the sub-corpora are independent, we have 
        \begin{equation}
            \mathbb{E}\frac{m_n(v, c)}{|\mathcal{D}_n|} = \mathbb{E}\frac{m_m(v, c)}{|\mathcal{D}_m|} \; \forall n, m 
        \end{equation}
        %\noident
        and hence 
        \begin{equation}
            \mathbb{E}\frac{m(v, c)}{|\mathcal{D}|} = \mathbb{E}\frac{m_n(v, c)}{|\mathcal{D}_n|} \; \forall n.
        \end{equation}

        In the remainder of the proof we can therefore focus on a corpus $\mathcal{D}_n$ generated by just a single random walk. We again denote with $v_j$ the $j$th vertex in this random walk generating~$\mathcal{D}_n$.

        The corpus $\mathcal{D}_n$ contains all the pairs $(w, c)$ such that for $0\leq j \leq L-T-1 \;\textnormal{and}\; 1\leq r\leq T$ either $(w = v_j, c = v_{j+r})$ or $(w = v_{j+r} , c = v_j)$ (cf. \Cref{algo:corpusgeneration}). 
        
        $\mathbb{E}\frac{m_n(w, c)}{|\mathcal{D}_n|}$ is the probability with which we would draw the pair $(w, c)$ from the corpus $\mathcal{D}_n$. Since $\mathcal{D}_n$ consists of the pairs from just a single (realisation of the) random walk $(v_i)_{0\leq i\leq L-1}$, 
        \begin{equation}
        \begin{split}
            \mathbb{P}(\textnormal{draw}\;&(w, c) \;\textnormal{from}\; \mathcal{D}_n) = \\
                &\mathbb{P}(\textnormal{draw}\;(w, c) \;\textnormal{from}\; (v_i)_{0\leq i\leq L-1}).
        \end{split}
        \end{equation} 
        
        The number of pairs $(v_i, v_j)$ in the corpus with $i > j$ is the same as the number of pairs with $i < j$. For a fixed start-vertex $s$, fixed $j$, and fixed $r$, the probability of drawing the vertex pair $(w, c)$ from the random walk therefore is
        \begin{align}
        \begin{split}
            \mathbb{P}(\textnormal{draw}\;&(w, c) \; | \; s, j, r) = \\
                &\frac{1}{2}[\mathbb{P}(w = v_j , c = v_{j+r} \; | \; s, j, r) \\
                &+ \;\mathbb{P}(w = v_{j+r} , c = v_j \; | \; s, j, r)].
        \end{split}
        \end{align}

        Also,
        \begin{alignat}{2}
            \mathbb{P}(w = v_j &, c = &&v_{j+r} \; | \; s, j, r) \\
                &= \;&&\mathbb{P}(w = v_j \; | \; s = v_0) \notag \\
                &\; &&\cdot \mathbb{P}(c = v_{j+r} \; | \; w = v_j, \; s = v_0) \label{proofeqn_1}\\[2ex]
            &= \; &&\mathbb{P}(w = v_j \; | \; s = v_0) \notag \\
            & \; &&\cdot \mathbb{P}(c = v_{j+r} \; | \; w = v_j) \label{proofeqn_2}\\[2ex]
            & = &&(P^j)_{sw} \cdot (P^r)_{wc}
        \end{alignat}
       %\noident
        where in going from \eqref{proofeqn_1} to \eqref{proofeqn_2} we used the Markov Property for the random walk $v_i$.
        We similarly obtain  
        \begin{equation}
            \mathbb{P}(w = v_{j+r}, c = v_j \; | \; s, j, r) = (P^j)_{sc} \cdot (P^r)_{cw}\;.
        \end{equation}

        The distributions of $j$ and $r$ are uniform (the number of pairs with some $j$, $r$ in $\mathcal{D}_n$ is the same for all $i, j$), so to evaluate the expectation values with respect to $j$ and $r$ we take the arithmetic mean. From \Cref{algo:corpusgeneration} we see that the distribution of $s$ is $f_{V_0}$, so the first part of the theorem follows.

        For the second part, note that $\frac{m(v, c)}{|\mathcal{D}|}$ is exactly the mean of the independent and identially distribution random variables  $\frac{m_n(v, c)}{|\mathcal{D}_n|}$, which take values in $[0,1]$. The law of large numbers therefore applies to show the almost sure convergence claimed.
    \end{IEEEproof}

    \begin{corollary}[Effect of Longer Random Walks]\label{cor:longerrandomwalks}
        Using the ergodic theorem (cf. Theorem 1.10.2 in \cite{norris1997markovchainsbook}), %and in particular \cref{cor_convtransitionmatrix}, 
        we can evaluate first the sum over $j$, and then the expectation value with respect to $s$, as $L\rightarrow \infty$.

        \begin{equation}\label{eqn:expectreloccurrenceconv}
            \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] \xrightarrow{a.s.} \; \frac{1}{2T}\sum_{r=1}^T \pi_v (P^r)_{vc} + \pi_c (P^r)_{cv}.
        \end{equation}

        Hence, as $N, L \rightarrow \infty$,
        \begin{equation}\label{eqn:reloccurrencesinfinitewalk}
            \frac{m(v, c)}{|\mathcal{D}|} \xrightarrow{a.s.} \; \frac{1}{2T}\sum_{r=1}^T \pi_v (P^r)_{vc} + \pi_c (P^r)_{cv}.
        \end{equation}
    \end{corollary} 
    \begin{remark}
        This almost sure convergence is stronger than the convergence in probability established in \cite{qiu2018unifying}. This is due to the fact that they do not let $N \rightarrow \infty$.
    \end{remark}

    \begin{corollary}[Effect of Starting Distribution]\label{cor:effectstartingdistr}
        From the definition of the stationary distribution we see that if $f_{V_0} = \pi$, 
        \begin{equation}
            \mathbb{E}_{s\sim f_{V_0}} (P^j)_{sv} = \pi_v.
        \end{equation}
        In that case, \eqref{eqn:expectreloccurrenceconv} holds as an equality for arbitrary $L>T$, and \eqref{eqn:reloccurrencesinfinitewalk} holds for arbitrary fixed $L$ as $N\to \infty.$
    \end{corollary}
    
    The results from this section, together with \cref{thm:convvertexreps}, guarantee that if the DeepWalk algorithm performs enough and long enough random walks, the learned vertex representations converge in the sense of \cref{thm:convvertexreps}.
    
    
\subsection{Convergence Rates}\label{subsec:convrate}
    
    Let us first investigate the convergence rate as $N \rightarrow \infty$ for arbitrary $L$. 

    \begin{theorem}[Convergence Rate as $N\to \infty$]\label{thm:Nconvspeed}
        The convergence of \cref{thm:relpairoccurrence} satisfies the concentration bound
        \begin{equation}
            \mathbb{P}(\left|\frac{m(v, c)}{|\mathcal{D}|}- \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]\right| > \varepsilon) < 2 \exp(-2 N \varepsilon^2)
        \end{equation}
        %
        for $\varepsilon > 0$.

    \end{theorem}

    \begin{IEEEproof}
        Let again $m_n(v, c)$ be the multiplicity function of the corpus $\mathcal{D}_n$ generated from the $n$th random walk. Each random walk has the same length, so $N \cdot |\mathcal{D}_n| = |\mathcal{D}| \forall n < N$. Since $0 \leq m_n(v, c) \leq |\mathcal{D}_n|$, Hoeffding's inequality gives
        \begin{equation}
        \begin{split}
            \mathbb{P}\left(\left|\sum_{n=1}^N m_n(v, c) - \mathbb{E}[\sum_{n=1}^N m_n(v, c)]\right| > \varepsilon\right) \\
            < 2 \exp\left(-\frac{2 \varepsilon^2}{N |\mathcal{D}_n|^2}\right).
        \end{split}
        \end{equation}
        
        Dividing by $|\mathcal{D}| = N |\mathcal{D}_n|$ and using $\sum_{n=1}^N m_n(v, c) = m(v, c)$ then yields
        \begin{equation}
        \begin{split}
             \mathbb{P}\left(\left|\frac{m(v, c)}{|\mathcal{D}|}- \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]\right| > \frac{\varepsilon}{N |\mathcal{D}_n|}\right) \\
            < 2 \exp\left(-\frac{2 \varepsilon^2}{N |\mathcal{D}_n|^2}\right).
        \end{split}
        \end{equation}
        Re-scaling $\varepsilon \to N |\mathcal{D}_n| \varepsilon$ then yields the theorem. 
    \end{IEEEproof}
    %We remark that a much finer estimate could be obtained here, as the variance in a typical edge $\sigma^2(v,c)$ is likely much less than $1$; such an effect may be important depending on the choice of norm on the space of matrixes. However, quantifying this relies largely on features of the specific graph to constrain the properties of the transition matrix $P$. 
    %We did not yet quantify the variance of the random variable $\frac{m_i(v, c)}{|\mathcal{D}_i|}$. 

    %Let us define the shorthand $\mathcal{I}_{j, r}(v, c) =  \mathbf{1}\{w_j = v, w_{j+r} = c\}$, where $w_i$ is the vertex in the $i$th step of the random walk. The variance can be calculated using $\mathbb{E}(\frac{m_i(v, c)}{|\mathcal{D}_i|})$ from \cref{thm_relpairoccurrence} and $\mathbb{E}(\left[\frac{m_i(v, c)}{|\mathcal{D}_i|}\right]^2)$. Writing
    %\begin{equation}
        %\frac{m(v, c)}{|\mathcal{D}|} = \frac{1}{L-T}\frac{1}{2T}\sum_{j=0}^{L-T-1} \sum_{r=1}^T %\mathcal{I}_{j, r}(v, c) + \mathcal{I}_{j, r}(c, v),
    %\end{equation}
    %we can use the fact that, assuming $k > j+r$,
    %\begin{align}
        %\mathbb{E}(\mathcal{I}_{j, r}(v, c) \cdot \mathcal{I}_{k, u}(v', c')) &= \mathbb{P}(w_j = v, w_{j+r} = c, w_k = v', w_{k+u} = c') \\
        %&= (P^j)_{sv} (P^r)_{vc} (P^{k-j-r})_{cv'} (P^s)_{v'c'}
    %\end{align}
    %to then in principle express the variance of $\frac{m(v, c)}{|\mathcal{D}|}$ solely in terms of the transition matrix $P$. However, doing this explicitly is not very enlightening, as any results heavily depend on the specific graph to constrain the values of the transition matrix $P$.

    To derive a concentration bound for the joint limit, we first need to prove two lemmas that quantify the convergence rate of $\mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]$ as $L\to \infty$ for undirected and directed graphs. For notational simplicity, define
    \begin{equation*}
        \omega(v, c) := \frac{1}{2T}\sum_{r=1}^T \pi_v (P^r)_{vc} + \pi_c (P^r)_{cv}
    \end{equation*}
    as the value that $\mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]$ converges to (\Cref{thm:relpairoccurrence}).

    %\subsubsection*{Undirected Graphs}

    \begin{lemma}[Convergence Rate for Undirected Graphs]\label{lemma:speedconvundirgraph}
        Given an undirected graph, let $d_i=\sum_j w_{ij}$ be the out-degrees and $D=\text{diag}(d_i)$. Let $\{\lambda_k\}$ be the ordered eigenvalues of the symmetric normalised graph Laplacian $$ L^\text{norm}=I-D^{1/2}PD^{-1/2}. $$ Then we have the convergence estimate
        \begin{equation*}
            \begin{split}
            \bigg|\mathbb{E}\bigg[&\frac{m(v, c)}{|\mathcal{D}|}\bigg] -  \omega(v, c)\bigg| \\
                &\leq \frac{1}{L-T} \frac{1-\phi_\star^{L-T}}{1-\phi_\star} \mathbb{E}_{s \sim f_{V_0}}\left[d_s^{-\frac{1}{2}}\right] \\
            &\;\;\;\;\cdot \frac{1}{2T} \sum_{r=1}^T \sqrt{d_v}(P^r)_{vc} + \sqrt{d_c}(P^r)_{cv} = O\left(\frac{1}{L}\right)
            \end{split}
        \end{equation*}
    where $\phi_\star \equiv \mu_\star = \sup\{|1-\lambda_2|, |1-\lambda_{|V|}|\}$ for non-bipartite graphs and $\phi_\star \equiv \nu_\star = \sup\{|1-\lambda_2|, |1-\lambda_{|V|-1}|\}$ for bipartite graphs and even $L-T$.
    \end{lemma}
    \begin{IEEEproof}\renewcommand{\qedsymbol}{}
        For a general undirected graph, we get by substituting for $\omega(v, c)$ and from \cref{thm:relpairoccurrence} for $ \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]$
        %
        \begin{alignat}{2}
            \bigg|\mathbb{E}\bigg[&\frac{m(v, c)}{|\mathcal{D}|}\bigg] -  \omega(v, c)\bigg| \notag \\
                &= \frac{1}{2T}| \mathbb{E}_{s \sim f_{V_0}} \mathbb{E}_j &&\sum_{r=1}^T [(P^j)_{sv} - \pi_v](P^r)_{vc} \notag \\
            &  \;&&+ [(P^j)_{sc} - \pi_c](P^r)_{cv} | \\
            &\leq \frac{1}{2T}\mathbb{E}_{s \sim f_{V_0}} \sum_{r=1}^T &&\left|\mathbb{E}_j(P^j)_{sv} - \pi_v\right|(P^r)_{vc} \notag \\
            & \qquad \qquad \qquad+&&\left|\mathbb{E}_j(P^j)_{sc} - \pi_c\right|(P^r)_{cv} \label{eqn:errorandepsmixingtime}
        \end{alignat}
        by Jensen's inequality. 
        For non-bipartite graphs, we again apply Jensen's inequality and use Theorem 5.1 in \cite{lovasz1993randomwalkssurvey} to obtain
        \begin{align}
            \mathrm{LHS} &\leq \frac{1}{2T}\mathbb{E}_{s \sim f_{V_0}}\mathbb{E}_j \sum_{r=1}^T \sqrt{\frac{d_v}{d_s}}\mu_\star^j (P^r)_{vc} \notag \\
                &\qquad \qquad \qquad \qquad+ \sqrt{\frac{d_c}{d_s}}\mu_\star^j (P^r)_{cv} \\[2ex]
            &\leq \frac{1}{L-T} \frac{1-\mu_\star^{L-T}}{1-\mu_\star} \mathbb{E}_{s \sim f_{V_0}}\left[d_s^{-\frac{1}{2}}\right] \notag\\ 
                &\qquad \cdot \frac{1}{2T} \sum_{r=1}^T \sqrt{d_v}(P^r)_{vc} + \sqrt{d_c}(P^r)_{cv} 
        \end{align}

        For $L-T$ even (so that $\mathbb{E}_j$ contains an even number of terms) for bipartite graphs, we replace $\mu_\star$ with $\nu_\star$, where the difference between the two stems from the fact that $1-\lambda_{|V|}=-1$, so in the derivation of Theorem 5.1 in \cite{lovasz1993randomwalkssurvey} successive terms involving $(1-\lambda_{|V|})^t$ cancel. The Lemma then follows.% \hspace{4cm}$\square$ \vspace{-1cm}

        %\begin{align}
           % LHS &\leq \frac{1}{2T}\mathbb{E}_{s \sim f_{V_0}} \sum_{r=1}^T \sqrt{\frac{d_v}{d_s}}\;\mathbb{E}_j \left[\nu_\star^j \right] (P^r)_{vc} \notag \\
          %      & \qquad \qquad \qquad + \sqrt{\frac{d_c}{d_s}}\;\mathbb{E}_j \left[\nu_\star^j \right] (P^r)_{cv} \\[2ex]
         %   &\leq \frac{1}{L-T} \frac{1-\nu_\star^{L-T}}{1-\nu_\star} \mathbb{E}_{s \sim f_{V_0}}\left[d_s^{-\frac{1}{2}}\right] \notag \\
        %        & \qquad \cdot\frac{1}{2T} \sum_{r=1}^T \sqrt{d_v}(P^r)_{vc} + \sqrt{d_c}(P^r)_{cv} 
        %\end{align}
        %The theorem follows.
    \end{IEEEproof}
    

        %We see that for undirected graphs, the speed of convergence of the expected value of the pair occurrence frequencies is $O\left(\frac{1}{L}\right)$.
        
        %We also see that the absolute value of the error is smaller for $(v, c)$ pairs where both vertices have small degrees and/or the random walk is unlikely to move from $v$ to $c$ and vice versa within $T$ steps. This is because such vertex pairs appear in the corpus less often in the first place. %In fact, because 
        
        %\begin{align}
        %    \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] &\sim \pi_v (P^r)_{vc} + \pi_c (P^r)_{cv} \\
        %    &\sim d_v (P^r)_{vc} + d_c (P^r)_{cv}
        %\end{align}

        %whereas the error is 
        %\begin{equation}
        %    \left|\mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] -  \omega(v, c)\right| \sim  \sqrt{d_v} (P^r)_{vc} + \sqrt{d_c} (P^r)_{cv}, 
        %\end{equation}
        %the error is larger for vertex pairs that appear less frequently than might be expected based on 5their occurrence frequency alone. 
%
%\subsubsection*{Directed Graphs}

    %Even for aperiodic directed graphs, we cannot use \cref{prop_transprobseigenvalueconnection}, and hence \cref{lemma_boundonabsolutevalue} and \cref{lemma_bipartitegraphconvergence}, because their adjacency matrices are not symmetric. 

    %Instead, we need to fall back on \cref{thm_convergencetheorem}. 

    \begin{lemma}[Convergence Rate for Directed Graphs]\label{lemma:speedconvdirgraph}
        For a directed graph $G$ with period $\Theta\geq 1$,
        \begin{equation}
            \left|\mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] -  \omega(v, c)\right| = O\left(\frac{1}{L}\right).
        \end{equation}
        Furthermore, if $G$ is aperiodic ($\Theta =1$), with constants $C$ and $\alpha \in (0, 1)$ as in Theorem 4.9 in \cite{levin2017markovmixing}, 
        \begin{align}\label{eqn:aperdirgraphconverror}
            &\left|\mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] -  \omega(v, c)\right| \notag \\
                &\qquad \leq \frac{C}{L-T} \frac{1-\alpha^{L-T}}{1-\alpha} \frac{1}{2T}\sum_{r=1}^T(P^r)_{vc} + (P^r)_{cv}.
        \end{align}
    \end{lemma}

    To prove this for both aperiodic and periodic graphs, we need the following intermediate result.
    \begin{proposition}\label{prop:periodicchainconv}
        Let $P$ be the transition matrix of a Markov chain $\{X_t\}_{t\geq 0}$ with period $\Theta$ and stationary distribution $\pi$. Let $\{\mathcal{S}_i\}_{1\leq i\leq \Theta}$ be the disjoint subsets of the state space $S$ such that $\mathbb{P}(X_{t+1}\in \mathcal{S}_{(i+1)\mod{\Theta}}|X_t \in \mathcal{S}_i)$. If vertices $s, v \in \mathcal{S}_i$ for some $i$, then there exist (explicitable) constants $\alpha \in (0, 1), \; C > 0$ such that
        \begin{equation*}
            \left|(P^{\Theta\cdot t})_{sv} - \Theta \cdot \pi_v \right| \leq C \alpha^t.
        \end{equation*}
    \end{proposition}
    \begin{IEEEproof}
       A similar observation is well-known for Markov chains in general (Theorem 4.9, \cite{levin2017markovmixing}); in the present context, it suffices to observe that $P^\Theta|_{\mathcal{S}_i}$ is an aperiodic stochastic matrix on the block $\mathcal{S}_i$, for which $\Theta \pi|_{\mathcal{S}_i}$ is an invariant probability measure, and the lemma follows from the cited result.   
       
       
       %\iffalse OLD Let us write $\mathcal{U}_i$ for the subspace of probability measures on $\mathcal{S}$ with support $\mathcal{S}_i$. Consider the restriction of matrix $P^\Theta$ to $\mathcal{U}_i$, denoted $P^\Theta|_{\mathcal{U}_i}$, and note that if  $(P^{\Theta\cdot t})_{sv} = ((P^\Theta|_{\mathcal{U}_i})^t)_{sv}$ if both $s,v\in \mathcal{S}_i$, and $=0$ if $s\in \mathcal{S}_i, v\not\in \mathcal{S}_i$ by periodicity; in particular it follows that $P^\Theta_{\mathcal{U}_i}$ is a stochastic matrix, which is aperiodic by construction. We can therefore define a new Markov Chain with state space $\mathcal{S}_i$, transition matrix $P^\Theta|_{\mathcal{U}_i}$, and stationary distribution $\pi|_{\mathcal{U}_i}$. 
        
        %Since the original Markov chain visits $\mathcal{S}_i$ every $\Theta$ steps, it follows from the Ergodic Theorem (Theorem 1.10.2 in \cite{norris1997markovchainsbook}) that the stationary distributions $\pi$ and $\pi|_{\mathcal{U}_i}$ are related by $ \pi|_{\mathcal{U}_i} = \Theta \cdot \pi.$ We can now apply Theorem 4.9 in \cite{levin2017markovmixing} to the new Markov chain to obtain the proposition. \fi
    \end{IEEEproof}
    With this proposition in hand, we are now in a position to prove the Lemma.
    \setcounter{theorem}{7}
    \begin{IEEEproof}[Proof of \Cref{lemma:speedconvdirgraph}]
        Substituting for $\omega(v, c)$ and from \Cref{thm:relpairoccurrence}  for $ \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]$ and using Jensen's inequality as in the proof for \Cref{lemma:speedconvundirgraph} again leads to  \eqref{eqn:errorandepsmixingtime}.

        We prove the first part of the theorem by showing that for a general periodic graph $\left|\mathbb{E}_j(P^j)_{sv} - \pi_v\right| = O\left(\frac{1}{L}\right)$.

        Let again $\{\mathcal{S}_i\}_{1\leq i\leq \Theta}$ be disjoint subsets of the state space $S$ as in \Cref{prop:periodicchainconv}. Without loss of generality, take $s \in \mathcal{S}_i$ and $v \in \mathcal{S}_k$ with $k \geq i$, and let $a = k -i$ so that $\sum_{s' \in \mathcal{S}_k} (P^a)_{ss'} = 1$. We decompose the path from $s$ to $v$ in $j$ steps, $(P^j)_{sv}$, into a part from $s\in \mathcal{S}_i$ to an $s' \in \mathcal{S}_k$ and a part from $s'\in \mathcal{S}_k$ to $v \in \mathcal{S}_k$: %\vspace{-0.4cm}
        \begin{align}
            \mathbb{E}_j(P^j)_{sv} &= \frac{1}{L-T}\sum_{j=0}^{L-T-1}(P^j)_{sv}\\
            %&= \frac{1}{L-T}\sum_{j=0}^{L-T-1} \sum_{s' \in \mathcal{S}_k} (P^a)_{ss'} (P^{j-a})_{s'v} \\
            &= \frac{1}{L-T}\sum_{j=a}^{L-T-1} \sum_{s' \in \mathcal{S}_k} (P^a)_{ss'} (P^{j-a})_{s'v} \\
            &= \frac{1}{L-T}\sum_{n=0}^{\lfloor \frac{L-T-a-1}{\Theta}\rfloor } (P^{\Theta \cdot n})_{s'v}
        \end{align}
        since if $j < a$ then $(P^j)_{sv} = 0$, and if $(j-a)\bmod \Theta \neq 0$ then $(P^{j-a})_{s'v} =0$, and since $\sum_{s' \in \mathcal{S}_k} (P^a)_{ss'} = 1$. We can use \Cref{prop:periodicchainconv} to obtain upper and lower bounds for $(P^{\Theta \cdot n})_{s'v}$
        \begin{equation}
            \Theta\cdot\pi_v - C \alpha^n \leq (P^{\Theta \cdot n})_{s'v} \leq \Theta\cdot\pi_v + C \alpha^n
        \end{equation}
        for some constants $C$ and $\alpha \in (0, 1)$.
        %\bigbreak
        %
        If $\mathbb{E}_j(P^j)_{sv} - \pi_v \geq 0$, we use the upper bound on $(P^{\Theta \cdot n})_{s'v}$, and if $\mathbb{E}_j(P^j)_{sv} - \pi_v \leq 0$ we use the lower bound to obtain:
        \begin{align}
            \mathrm{LHS} \leq &\left| \frac{1}{L-T}\sum_{n=0}^{\lfloor \frac{L-T-a-1}{\Theta}\rfloor} (\Theta\cdot\pi_v)- \pi_v\right| \notag \\
            &+ \frac{1}{L-T}\sum_{n=0}^{\lfloor \frac{L-T-a-1}{\Theta}\rfloor} (C\alpha^n).
        \end{align}
        %
        Using the fact that $\left\lfloor \frac{x}{y} \right\rfloor = \frac{x}{y} - \frac{x\bmod y}{y}$ to evaluate the prefactor of $\pi_v$, we continue
        \begin{alignat}{2}
            \mathrm{LHS} &\leq &&\left|\frac{\Theta}{L-T} \left(\left\lfloor \frac{L-T-a-1}{\Theta}\right\rfloor + 1\right) -1 \right| \pi_v \notag \\
            & &&+ \frac{1}{L-T}\sum_{n=0}^{\lfloor \frac{L-T-a-1}{\Theta}\rfloor} C \alpha^n \\
            &\leq &&\left|\frac{\Theta - a - 1 - (L-T-a-1)\bmod \Theta}{L-T} \right| \cdot\pi_v \notag \\
            & && + \frac{1}{L-T}\sum_{n=0}^{\lfloor \frac{L-T-a-1}{\Theta}\rfloor} C \alpha^n \label{eqn:periodicgraphbound} \\
            &= && \;O\left(\frac{1}{L}\right)
        \end{alignat}
        since the remaining geometric sum is bounded by a constant.
        
        To prove the second part of the theorem, note that for aperiodic graphs, $\Theta = 1$ and $i=k \Rightarrow a = 0$. For aperiodic graphs, $C$ and $\alpha$ still have the same meaning as before. 

        Therefore, in \eqref{eqn:periodicgraphbound} the prefactor of $\pi_v$ vanishes for aperiodic graphs. The upper bound on $\left|\mathbb{E}_j(P^j)_{sv} - \pi_v \right|$  therefore evaluates to
        \begin{align}
            \left|\mathbb{E}_j(P^j)_{sv} - \pi_v \right| &\leq \frac{C}{L-T} \sum_{n=0}^{L-T-1}\alpha^n \\
            &\leq \frac{C}{L-T} \frac{1-\alpha^{L-T}}{1-\alpha}.
        \end{align}
        Substituting into \eqref{eqn:errorandepsmixingtime}, the theorem follows.
    \end{IEEEproof}
    \setcounter{theorem}{5}
    
    Finally we state and prove our theorem for the convergence rate in the joint limit $N, L \to \infty$:
    \begin{theorem}[Convergence Rate as $N, L\to \infty$]\label{thm:jointconvrate}
        The convergence of \cref{cor:longerrandomwalks} satisfies the concentration bound
        \begin{equation}
            \mathbb{P}\left(\left|\frac{m(v, c)}{|\mathcal{D}|} - \omega(v, c)\right| > \varepsilon\right) < 2 \exp(-2N(\varepsilon - U)^2)
        \end{equation}
        for $\varepsilon>U >0$, and where $U$ is the appropriate upper bound for $\bigg|\mathbb{E}\bigg[\frac{m(v, c)}{|\mathcal{D}|}\bigg] -  \omega(v, c)\bigg|$ as derived in lemmas \ref{lemma:speedconvundirgraph} and \ref{lemma:speedconvdirgraph} and depends only on $L, T$, and graph-specific constants.
    \end{theorem}
    
    \begin{IEEEproof}
        We have by the triangle inequality 
        
        \begin{align}
        \begin{split}
            &\left|\frac{m(v, c)}{|\mathcal{D}|}- \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]\right| \notag \\
                &\;\;\;\;\geq \left|\frac{m(v, c)}{|\mathcal{D}|}- \omega(v, c)\right| - \left| \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] - \omega(v, c)\right|.
        \end{split}
        \end{align} 
        
        Therefore, 
        
        \begin{align}
        \begin{split}
            \mathbb{P}&\left(\left|\frac{m(v, c)}{|\mathcal{D}|}- \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right]\right| > \varepsilon \right) \notag \\
                &\geq \mathbb{P}\left(\left|\frac{m(v, c)}{|\mathcal{D}|}- \omega(v, c)\right| - \left| \mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] - \omega(v, c)\right| > \varepsilon \right) \\
                & = \mathbb{P}\left(\left|\frac{m(v, c)}{|\mathcal{D}|}- \omega(v, c)\right| > \varepsilon + \left|\mathbb{E}\left[\frac{m(v, c)}{|\mathcal{D}|}\right] - \omega(v, c)\right|\right) \\
                & \geq \mathbb{P}\left(\left|\frac{m(v, c)}{|\mathcal{D}|}- \omega(v, c)\right| > \varepsilon + U\right).
        \end{split}
        \end{align}
        
        Substituting $\varepsilon \to \varepsilon - U$ and using \Cref{thm:Nconvspeed} then yields the result.
    \end{IEEEproof}

    % Old prose{
        %In principle we could also write down an equation similar to \ref{eqn:aperdirgraphconverror} for periodic graphs, in which case we would retain the terms involving $\pi_v$ whose sign depends on the sign of $\mathbb{E}_j(P^j)_{sv} - \pi_v$.

        %For most vertex pairs this upper bound is clearly looser than the one we derived for undirected graphs, since $C$ and $\alpha$ do not depend on the vertex pair for which we bound the error.
        %\bigbreak
        %We see that the convergence rate of the expected value of the vertex pair occurrence frequencies is $O\left(\frac{1}{L}\right)$ for all types of (irreducible) graphs as the length of the random walks $L$ increases.
        %\bigbreak
        %A detailed investigation of the remaining open question, the behaviour of the variance of $\frac{m(v, c)}{|\mathcal{D}|}$ as $L\rightarrow \infty$ but with $N$ finite, would not be possible without moving beyond the scope of this essay. 
        
        %I nevertheless conjecture that at least if the distribution of the start vertex is the stationary distribution, the variance scales as $O\left(\frac{1}{L}\right)$ and the standard deviation as $O\left(\frac{1}{\sqrt{L}}\right)$. 
    
        %This is based on the intuition that with this start vertex distribution, one can partition each long random walk of length $L$ into $M = \frac{L}{\mathcal{L}}$ shorter random walks of length $\mathcal{L}$ that too have their start vertices distributed according to the stationary distribution. As $L \rightarrow \infty$ with $\mathcal{L}$ fixed, we have $M \rightarrow \infty$, and we can use the Central Limit Theorem as in \cref{cor_Nconvspeed} together with $M \propto L$.}
    
    We can use \Cref{thm:jointconvrate} to obtain a rough heuristic for an "optimal" choice of the parameters $N$ and $L$ given a fixed computational cost; the window size $T$ determines the size of the local structures which the vertex embeddings encode and is therefore usually fixed for a given application. The total computational cost of computing the co-occurrence matrix scales linearly with the number of random-walk steps $N \cdot L$, but since $L\geq T$ we define the \textit{excess computational cost} $K = N \cdot L - N \cdot T = N \cdot (L-T)$. 
    
    For notational simplicity we also denote the upper bound for the failure probability in \Cref{thm:jointconvrate} as $\delta = 2 \exp(-2N(\varepsilon - U)^2)$ and absorb all terms in $U$ that are independent of $N, L$ into a constant $g$ for notational simplicity. Then we have:
    
    \begin{corollary}\label{cor:heuristic}
        Assuming that $K \gg N$ so that $\phi^{K/N} \approx 0$ and $\alpha^{K/N} \approx 0$ in $U$, the value for $N$ that minimises the error $\varepsilon = U + \sqrt{\frac{1}{2N}\log{\frac{2}{\delta}}}$ given $K, \delta$ fixed is
        \begin{equation}
            N \approx \frac{1}{2}\sqrt[3]{\frac{K^2}{g^2}\log{\frac{2}{\delta}}}.
        \end{equation}
    \end{corollary}
    This heuristic minimises the error $\varepsilon$ given an excess computational cost $K$ and an upper bound for the failure probability $\delta$, which both can be freely chosen.
    We see that under the heuristic, $N = O\left(K^{\frac{2}{3}}\right)$, which justifies the assumption $K \gg N$. Even without this assumption, we still have an upper bound, as the neglected terms $-\phi^{K/N}, -\alpha^{K/N}$ can only make $\varepsilon$ smaller. 
    In practice, one could use $g \approx 1$ as a first approximation to the remaining constant $g$, which depends on the graph structure through the spectrum or through $\alpha$. If a more precise estimate for $g$ is needed, let us remark that this proof (and the results recalled in the Appendix) produce a construct\emph{able} $g$, in that one can follow the steps of the proofs to explicitly find $g$ for a given example. In the case where we use \Cref{lemma:speedconvundirgraph}, let us remark that many techniques are known (\cite{diaconis1991geometric}, and references therein) for bounding spectral gaps, which would lead to a constructable upper bound for $g$. 
    
    

\subsection{Convergence of Vertex Representations}\label{subsec:convvertexreps}
    We finally show that convergence of the corpora, suitably normalised, is indeed sufficient to show convergence of the vertex representations.

%In order to propagate the convergence to the vertex embeddings, we assume that the map \begin{equation} \label{assumption:optimcontinuity} f\mapsto f(A(f)) \text{ is continuous} \end{equation} on some space of objective functions $f\in F$, with respect to the essential supremum distance $\|\cdot\|_\infty.$

    We first remark that, if two corpora $\mathcal{D}^i=(D^{(i)},m^{(i)}), i=1,2$ differ only by a constant multiple so that $$ D^{(1)}=D^{(2)}; \qquad m^{(1)}=c\cdot m^{(2)} $$ for some $c>0$, then the respective partial applications of the objective function also differ only up to a constant multiple: $f^{(1)}=cf^{(2)}$, and it follows that the derived vertex embeddings \begin{equation} \label{lemma:equalrepresentationssufficientcondition} \{z^{(1)}_i\}_{i:\;v_i \in V} =\{z^{(2)}_i\}_{i:\;v_i \in V}\end{equation} also agree. To remove this redundancy, we define normalised objective functions
    \begin{equation}
        f^{\textrm{norm}} = \frac{1}{|\mathcal{D}|}\cdot f. \label{eqn:normalisedobjfunctiondefn}
    \end{equation}
    By \eqref{lemma:equalrepresentationssufficientcondition} this normalisation does not change the learned representations.
    
    We next assume the following:
    \begin{assumption}\label{assumption:objfunction}
        The objective function is of the same form as in~\eqref{assumption:objfunctionform}, with the $g_{ic}$ bounded.
    \end{assumption}
    \begin{assumption}\label{assumption:optimcontinuity} 
        The map 
        \begin{equation}        
            f\mapsto f(A(f)) \text{ is continuous} 
        \end{equation} on some space of partial applications of objective functions, with respect to the essential supremum distance $\|\cdot\|_\infty$, where $A$ is the optimisation procedure $A: f \mapsto \mathcal{X}$ as before.
    \end{assumption}
    Informally, \Cref{assumption:optimcontinuity} means that if the partial application of the objective function, $f$, changes slightly, the optimisation procedure will find vertex embeddings that have a similar objective value.

    \begin{theorem}[Convergence of Vertex Representations]\label{thm:convvertexreps}
        Let $(\mathcal{D}_n)$ be a sequence of corpora generated by \Cref{algo:corpusgeneration} from the same graph such that the respective vertex pair occurrence frequencies $\left(\frac{m_n}{|\mathcal{D}_n|}\right)$ converge to the vertex pair occurrence frequencies $\frac{m}{|\mathcal{D}|}$ in some corpus $\mathcal{D}$ generated from that graph. Let $f_n$ be the partial application of an objective function given corpus $\mathcal{D}_n$, and $f^{\textnormal{norm}}_n$ the normalised objective function, and similarly define $f$ and $f^{\textnormal{norm}}$; . Then 
        \begin{equation*}
            f^{\textnormal{norm}}_n(A(f_n)) \longrightarrow f^{\textnormal{norm}}(A(f)).
        \end{equation*}
    \end{theorem}
   

    
    \begin{IEEEproof}
        The map $\frac{m(\cdot)}{\mathcal{D}}\to f^\textrm{norm}$ is continuous with respect to the uniform distance on functions, as the $g_{ic}$ are bounded.
        
        By continuity of $f^{\textrm{norm}}_n$ with respect to $\left(\frac{m_n}{|\mathcal{D}_n|}\right)$, $\left(\frac{m_n}{|\mathcal{D}_n|}\right) \rightarrow \frac{m}{|\mathcal{D}|}$ implies $f^{\textrm{norm}}_n \rightarrow f^{\textrm{norm}}$.

        By continuity of $f^{\textrm{norm}}_n(A(f^{\textrm{norm}}_n))$ with respect to $f^{\textrm{norm}}_n$, $f^{\textrm{norm}}_n \rightarrow f^{\textrm{norm}}$ implies  $f^{\textrm{norm}}_n(A(f^{\textrm{norm}}_n)) \rightarrow f^{\textrm{norm}}(A(f^{\textrm{norm}}))$.

        From~\eqref{lemma:equalrepresentationssufficientcondition} we know that $A(f^{\textrm{norm}}_n) = A(f_n)$ and $A(f^{\textrm{norm}}) = A(f)$ and the theorem follows.
    \end{IEEEproof}

    \Cref{thm:convvertexreps} means that if the vertex pair occurrence frequencies of $(\textnormal{vertex}, \textnormal{context})$ pairs converge to those of some corpus $\mathcal{D}$, then the vertex representations converge to values that have the same (normalised) objective function value as the representations derived from corpus $\mathcal{D}$ and should be similarly useful for downstream tasks.
    
  

==> LaTeX Source/sections/experiments.tex <==
\section{Experimental Results}\label{sec:experiments}
In this section, we detail the set of experiments that we conducted to illustrate our theoretical findings. 
%\Angie{Will update the details in the text once all plots are done}

\begin{table}[t!]
\caption{Characteristics of the datasets used in our experiments.}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{cccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\textsc{Dataset} & \begin{tabular}[c]{@{}c@{}}\#  \textsc{of }\\ Classes\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\# \textsc{of Nodes}\\ $|V|$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\# \textsc{of Edges}\\ $|E|$\end{tabular} \\ \hline
\textsc{Cora} & 7 & 2,708 & 5,429 \\
\textsc{BlogCatalog} & 39 & 10,312 & 333,983 \\
\textsc{Wiki} & 19 & 2,405 & 17,981 \\
\textsc{Facebook Large} & 4 & 22,470 & 171,002 \\
\textsc{Youtube} & 47 & 1.1M & 4.9M \\ \hline
\end{tabular}
}
\label{table:datasets}
 %\vspace{-0.5cm}
\end{table}

\begin{figure}[t!]  
	%\begin{centering}
		\includegraphics[width=1\linewidth]{./Figs/Graphs.pdf}\vspace{-0.3cm}
		%\end{centering}
		\vspace{-0.2cm}
	\caption{Graph visual representation of some of the datasets used in our experimental results. } \label{fig:Graphs}
\end{figure}


\begin{figure*}[t!]
\begin{minipage}[b]{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/Convergence2.pdf}
            \caption{Convergence of co-occurrence matrices as the trajectory length $L$ and the number of walks $N$ approach infinity. The error is the computed as $\Vert m - \omega\Vert_2$, and we use $N=80$ when varying $L$ and $L=40$ when varying $N$. }
            \label{fig:matrixconvergence}
        \end{minipage}
        \hspace{0.1cm}
        \begin{minipage}[b]{0.49\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/K_Last2.pdf}
            \caption{Computational cost in the x-axis expressed as  $K =  N \cdot (L-T)$ against the task performance, in terms of Micro-F1, on the y-axis. The plots compare our derived heuristic with two other cases where the parameters are not optimal.}
            \label{fig:heuristic}
\end{minipage}
\end{figure*}

\begin{figure*}[t!]  %% teaser figure for the paper
	\begin{centering}
		\includegraphics[width=1\linewidth]{./Figs/MainResults.pdf}
		\par\end{centering}
	\caption{Performance on a classification task for different using embeddings generated with different hyperparameter choices for the number of random walks $N$, the length of each random walk $L$, and the embedding dimension $d$. We use $N=80$ when varying $L$ and $L=40$ when varying $N$, and fix $d=128$ for plots (c)-(f).} \label{fig:taskperformanceconvergence}
\end{figure*}

%\& Evaluation Protocol
\subsection{Datasets Description}~\label{exp:eval}
We used five real-world datasets for our experiments. Each is a graph whose vertices are grouped in a number of classes. They vary in their number of nodes and edges (up to the order of millions) and in their number of classes. The dataset statistics are given in \Cref{table:datasets} along with a graphical visualisation (see \cref{fig:Graphs}).
%
\begin{itemize}
    \item The \textsc{BlogCatalog}~\cite{tang2009relational} dataset is derived from a blog-sharing website. The edges reflect the bloggers (vertices) following each other. The classes in the dataset are the bloggers' interests. 
    \item The \textsc{Cora}~\cite{sen2008collective} dataset is a text classification dataset for Machine Learning papers. Each vertex corresponds to a paper with the edges representing citation links. The classes are different areas in Machine Learning. The dataset also supplies bag-of-word representations for each vertex, though we did not use these in our experiments.
    \item The \textsc{Wiki}~\cite{yang2015network} dataset, similarly to Cora, is a collection of text documents (vertices) with edges representing hyperlinks between them.
    \item The \textsc{Facebook Large}~\cite{rozemberczki2019multi} dataset is a page-page graph of Facebook sites. The vertices refer to Facebook pages while the edges denote mutual likes between sites.
    \item The \textsc{YouTube}~\cite{mislove2007measurement} dataset is based on the online video-sharing platform, with edges reflecting subscription connections between users (vertices). 
\end{itemize}


%\textbf{Evaluation Protocol.}
%We validate our theory using a three-parts evaluation scheme. 

%We validate our theory using the embeddings for multi-label classification.
%\smallskip

%We validate our theory using a three-parts evaluation scheme described next.



%\Angie{I moved the explanation of the experiments to the next section as the discussion might be longer in the main subsection 5.2}
% TODO Explain experiments here
% \textbf{(E1) Convergence of co-occurrence matrices.}
% We directly validate our results about the speed of convergence for the corpus generated by the first stage of DeepWalk (Theorems \ref{thm:Nconvspeed} and \ref{thm:jointconvrate}) as follows. %TODO
% We quantify the error of the co-occurrence matrix $M$ and the limit that it converge for different values of $N$ and $L$. More precisely, for all experiments run in this part we set $T=10$ and the dimension to 128. Moreover, for the effect of the number of walks we run 

%\textbf{(E2) Convergence of task performance.}

%TODO talk about how we can't easily measure convergence of embeddings directly because of the special notion of convergence that we assume, so we use task performance as a proxy

%\textbf{(E3) Heuristic for optimal values for $N$ and $L$.}

% talk about the heuristic and the experiments for that




%Following standard protocol in network embeddings, we reported the results using Micro-F1 metric. For all datasets, we set the windows size to $T=10$, and the embbeding dimension to 128, except for the \textsc{BlogCatalog} dataset where we report the performance with embedding dimension sizes of 16, 128 and 256. For the classifier, we set the training ratio to 0.4 except for the \textsc{Youtube} dataset for which we use 10\%. To fulfill the goal of this work, we report a large range of values for the number of walks $N$ and the walk length $L$ from   $10^1$  to $10^6$ for the converge experiments,  and $2^0$  to $2^{10}$ for the task performance experiments. 
%Thirdly, to further elevate the relevance of our theoretical analysis, we support our derivation for optimal values for $N$ and $L$.
%Finally, we provided visual results for the generated embeddings along  a comparison of parameters vs  the wall-clock time related to the embeddings generation.   All test and comparison were run on a CPU-based implementation and coded in Python following~\cite{perozzi2014deepwalk}. 



% \begin{figure*}[t!]  %% teaser figure for the paper
% 	\begin{centering}
% 		\includegraphics[width=1\linewidth]{./Figs/EmbeddingsVisualisation.pdf}
% 		\par\end{centering}
% 	\caption{Parameters vs computational comparison using the \textsc{Cora} dataset. (From left to right) Illustration of a graph  classification output, where the colours denote different class labels. The different embeddings are obtained by varying the number and length of walks, resulting in varying Micro-F1 scores and elapsed wall-clock times.} \label{fig:exps2}
% \end{figure*}


\subsection{Results \& Discussion}
We support our theoretical analysis following a three-part evaluation scheme.


%we compared our derived heuristic for optimal values for the hyperparameters $N$ and $L$ against two other cases m

\smallskip
\textbf{(E1) Convergence of co-occurrence matrices.}
We begin by directly validating our results about the speed of convergence for the corpus generated by the first stage of DeepWalk (Theorems \ref{thm:Nconvspeed} and \ref{thm:jointconvrate}).%TODO

To do this, we calculate the approximation error of the co-occurrence matrix $m$ as the Frobenius norm of the difference between $m$ and its asymptotic value $\omega$, i.e. $\Vert m - \omega\Vert_2$, for different values of the random walk length $L$ and the number of random walks $N$.

More precisely, for all experiments run in this part we set the window size $T=10$ and the embedding dimension $d=128$. To observe the effect of increasing the number of walks, we set $N=\{10^1, 10^2, 10^3, 10^4, 10^5, 10^6\}$  and fix $L=40$ (see blue lines in \cref{fig:matrixconvergence}). The effect of increasing the length of the walk, we  set $L=\{10^1, 10^2, 10^3, 10^4, 10^5, 10^6\}$ and fix $N=80$ (see red lines in \cref{fig:matrixconvergence}). We ran these experiments using the \textsc{BlogCatalog} and \textsc{Cora} datasets. The results are displayed in \cref{fig:matrixconvergence}, where one can observe a convergence rate consistent with our results for the limiting cases when $N \to \infty$ and  $L \to \infty$.

%(a) and (b), we display the results where the $x$-axis display the trajectory for $L$ and $N$ while the $y$-axis is the quantified error of the co-occurrence matrix generated from the co-occurence matrix $M$ and the limit that the matrix converges. 
%We observe the behaviour discussed in our theoretical analysis -- that is,  the number of random walks $N$ goes to $\infty$ this convergence is almost sure both in the single limit $N \to \infty$ and the double limit $N, L \to \infty$.

%We experimentally support our theoretical analysis by a set of numerical experiments (\Cref{thm:relpairoccurrence}, \Cref{cor:longerrandomwalks}, \Cref{thm:Nconvspeed}, \Cref{thm:jointconvrate})using the BlogCatalog and Cora datasets. We set the trajectory for the number of walks and the length of the walks  in the range of \{$10^1, 10^2, 10^3, 10^4, 10^5, 10^6$ \}.  



\smallskip
\textbf{(E2) Heuristic for optimal values for $N$ and $L$.} We show the practical application of our heuristic for optimal choices of the hyperparameters $N$ and $L$ for a fixed computational complexity $K =  N \cdot (L-T)$ and fixed failure probability $\delta$ (\Cref{cor:heuristic}). 
For our experiments, we plot the task performance against the computational cost $K$ when choosing $N$ and $L$ using three different strategies. In the first strategy, we set $L = T + 1$ and $N = K$ to simulate the extreme of the minimum random walk length (red line in \cref{fig:heuristic}). In the second strategy, we set $N=1$ and $L = T + K$, the case of performing a single very long walk, which corresponds to the hyperparameter choice suggested in \cite{qiu2020matrix} (green line in \cref{fig:heuristic}). Finally, we select $N$ and $L$ using our heuristic, approximating the constant $g \approx 1$ and fixing $\delta = 0.01$ (blue line in \cref{fig:heuristic}).

The task performance is the Micro-F1 score achieved by the one-vs-rest logistic regression suggested by \cite{perozzi2014deepwalk} and also used in \cite{qiu2018unifying,qiu2020matrix}. For all strategies we again set $T=10$ and $d=128$. We ran these experiments using the \textsc{BlogCatalog} and the \textsc{Facebook Large} datasets for the values $K = \{2^{10}, 2^{11}, 2^{12}, 2^{13}, 2^{14}, 2^{15}\}$, so after necessary rounding the values used to test the heuristic were $N = \{88, 140, 224, 355, 563, 892\}$ and $L-T = \{12, 15, 18, 23, 29, 37\}$. The results are plotted in \cref{fig:heuristic}.

Choosing $N$ and $L$ using the heuristic consistently outperforms the other two cases, illustrating the impact that a better choice of the hyperparameters $N$ and $L$ can have. The maximally-parallelisable choice of $N=K$ and $L =T +1$ performs a lot worse than the other two strategies, which is likely due to the uniform starting distribution $f_{V_0}$ being too different to the stationary distribution on these graphs, resulting in the vertex contexts generated from the short walks not being very informative.



%For this experiment, we compared performance-wise our heuristic against two other cases. 
%More precisely, for the first case from $K =  N \cdot (L-T)$ we fix $N=1$ (see green line in Figure~\ref{fig:K_Last2}),  the second  case is the result from  fixing $L-T = 1$ (see red line in Figure~\ref{fig:K_Last2}). These two cases are compared against our heuristic given optimal values for $N$ and $L$ (see blue line in Figure~\ref{fig:K_Last2}). We ran these experiments using the \textsc{BlogCatalog} and the \textsc{Facebook Large} datasets.  We evaluate the range of $K = \{2^{10}, 2^{11}, 2^{12}, 2^{13}, 2^{14}, 2^{15}\}$ and using the Micro-F1 metric as performance evaluation. The comparisons are displayed in Figure~\ref{fig:K_Last2}. From the results we can observe that our derived heuristic,  \Cref{cor:heuristic}, fulfill its purpose and reported higher performance, for all the range of $K$, than the compared two cases. 

%Case 1 from $K =  N \cdot (L-T)$ we fix $N=1$, Case 2 is the result from  fixing $L-T = 1$ and Case 3 is our heuristic given optimal values for $N$ and $L$. 

%For this experiment, we use the BlogCatalog and Facebook Large datasets and set $K$ in the range of \{$2^{10}, ... , 2^{15}$\}. The results are displayed in Figure~\ref{fig:ExpLast} (c) and (d). We observe that our derived heuristic in \Cref{cor:heuristic} perform better than the other two cases for both  datasets and all range of $K$.


%Firstly, we support our theory by displaying the convergence of co-occurrence matrices as the number of walks $N$ and their length $L$ become infinite. 
%We show the experimentally the relation between the number of walks $N$

\textbf{(E3) Convergence of task performance.} In practice, vertex embeddings are seldom the final goal of a machine learning pipeline, and our notion of convergence in \cref{thm:convvertexreps} takes even two different sets of vertex embeddings to be equivalent if they result in the same (normalised) objective function value. We therefore use convergence of the task performance of a down-stream algorithm as a proxy for the convergence of the vertex embeddings; if the downstream task performance has converged then the vertex embeddings have very likely converged as well (in the sense of \cref{thm:convvertexreps}).

We again use the standard protocol for network embeddings evaluation (\cite{perozzi2014deepwalk,qiu2018unifying,qiu2020matrix}) and compute the Micro-F1 score of a one-vs-rest logistic regression.   
We again set the window size $T=10$. The results are plotted in \cref{fig:taskperformanceconvergence}. For the experiments in \cref{fig:taskperformanceconvergence} (a) and (b) we use varying embedding dimensions of $d = \{16, 128, 256\}$, while we keep the embedding dimension constant at $d=128$ for the other experiments in plots (c)-(f). When varying $L$, we set $N=80$, and when varying $N$, we set $L=40$.




%In Figure~\ref{fig:exps1}, we report the classification results in terms of the Micro-F1 metric. We run the experiments setting the dimension to 128 for plots (c)-(f) Figure~\ref{fig:exps1}, whilst setting the dimension to $\{16, 128, 256\}$ for plots (a)-(b). All experiments were evaluated varying $N$ and $L$ in the range of  $\{2^{0}, 2^{1}, 2^{2}, 2^{3}, ... , 2^{10}\}$ for plots (a)-(e), and $\{2^{5}, 2^{6}, 2^{8}, 2^{9}, 2^{10}\}$ for the YouTube dataset plot (f). We set $N=80$ when varying $L$ and  $L=40$ when varying $N$. 

One observes that as the number of walks and the length of each walk are tending to large values the performance converges. %For example, one can see a clear performance improvement between  the parameters values of $2^1$ and $2^5$. However,  $2^{10}$ does not offer a significant improvement over~$2^5$. 
%
This observation holds across all graph sizes and dimensions, for both medium-sized graphs like the \textsc{Cora} dataset and large graphs like the \textsc{BlogCatalog} dataset and embedding dimensions ranging from $d=16$ to $d=256$.

%and dimensions. example, the same flat region, in terms of performance from the plots in Figure~\ref{fig:exps1}, can be observed at large values for a medium size graph like the \textsc{Cora} dataset and a large graph such as the \textsc{Youtube} dataset. The results of changing the dimension size are displayed in Figure~\ref{fig:exps1} for the \textsc{BlogCatalog} dataset. We ran the same experiments under varying dimension of 16, 128 and 256. From the results, we can observe that the performance is stable as the parameters take large values, holds and that this stability is independent of the size dimension. 

%\textbf{(E4) Computational time vs Performance} To further support the practical implications of our theory, we evaluate the computational time vs performance when varying  the number of walks and the length of the walk. These results are displayed in Figure~\ref{fig:exps2}. From the results, we observe that obtaining meaningful embeddings is relevant for performance at the classification task at hand. The selection of very small or large values in the parameters leads to negative effects such as a degradation of the performance or substantial increments in the computational time (see first and third column from the embbedding plots). However, one can find a good trade-off between performance and computational time by selecting appropriate parameters (optimal parameters are discussed in point \textbf{(E2)}).


==> LaTeX Source/sections/formaldescription.tex <==
\section{Formal Description of the Deepwalk Algorithm} \label{sec:formaldeepwalkdescr}
    The DeepWalk algorithm consists of two phases: in the first phase it generates a corpus of vertex pairs, and in the second phase it executes the SkipGram algorithm (with negative sampling) on this corpus to generate vertex embeddings. 

\subsection{Generation of Corpus}

    Informally, in the first phase the corpus $\mathcal{D}$ is populated with all pairs of vertices that are within a given window size $T$ of each other in random walks generated on the graph. For each vertex, the vertices at most $T$ removed in the random walk are viewed as that vertex's \say{context} vertices, and each $(\textnormal{vertex},\; \textnormal{context vertex})$ pair is added to the corpus. 

    We take a graph $G=(V, E)$, equipped with a weight function $w:E\to [0,\infty)$.
    Consider a random walk $(V_t)_{t\ge 0}$ on $G$, with a given starting distribution $f_{V_0}$ and transition matrix $P$ with elements $P_{ij}=w_{ij}/\sum_j w_{ij}$, where $w_{ij}$ is the weight of edge $(v_i, v_j)$. We write $\textsc{Markov}(f_{V_0}, P, L)$ for the joint law of the first $L$ steps $(V_0, ...., V_{L-1})$ and, if $f_{V_0}=\delta_{v_0}$ is a one-hot distribution, write $\textsc{Markov}(v_0, P, L)$ instead. The stationary distribution of this random walk is denoted as $\pi \in \mathbb{R}^{|V|}$, which is given explicitly by $\pi(v_i)\propto\sum_j w_{ij}$.
        

    We define a \textit{corpus} $\mathcal{D}$ on graph $G=(V, E)$ to be a tuple $(D, m)$ consisting of the set of pairs $D = V \times V$ and the \textit{multiplicity function} $m: D \rightarrow \mathbb{N}$. Its \textit{cardinality} is the total multiplicity $|\mathcal{D}| =\sum_{d \in D} m(d)$. Since $|D|$ is finite, we may identify $m$ with the vector of its values, and write $m \in \mathbb{R}^{|V|\times|V|}_{\geq 0}$, and we denote its elements as $m(i, j) = m((v_i, v_j))$ for all $v_i, v_j \in V$, so for all $(v_i, v_j) \in D$. This matrix $m$ is also called the \textit{co-occurrence matrix}, as it encodes the number of co-occurrences of two vertices (the number of times the appear within $T$ random walk steps of each other) in the random walks performed. Note that once we have specified a graph, different corpora only differ in their multiplicity functions. 
        
    In the first phase of DeepWalk, an initially empty corpus is populated by repeatedly updating the multiplicity function. Formally, the algorithm with objective to populate the corpus $\mathcal{D}$ is given in Algorithm~\ref{algo:corpusgeneration}, taking as parameters the number of walks $N$, the walk length $L$ and window size $T$.
%
       
    In the second loop in line \ref{line:secondloop}, we follow \cite{qiu2018unifying} in having $j$ take on $L-T$ different values to avoid edge effects (when $j+r > L-1$). This simplifies the derivation in \cref{subsec:convrandomwalks} while only removing constant order terms (depending only on the fixed length $T$) from the equations.

\subsection{Generation of Vertex Representation}
    Having obtained a corpus in the first stage, in the second phase the vertex representations are calculated from the corpus. Traditionally using either the SkipGram algorithm~\cite{mikolov2013skipgram} or SkipGram with Negative Sampling~\cite{mikolov2013negativesampling} (though in principle other methods can be used as well), the vertex representations $\{z_i\}_{i:\;v_i \in V}$ are obtained by maximising an objective function of the form
    \begin{equation} \label{assumption:objfunctionform}
        F(Z, \mathcal{D}) = \sum_{(v_i, v_c)\in D} m((v_i, v_c))\cdot g_{ic}(Z)
    \end{equation}
    with respect to the $d\times|V|$ matrix $Z$. Here, $Z$ is the matrix of vertex embeddings whose columns are the individual $z_i$, $d$ is the dimension of each embedding, and $g_{ic}$ is some $g_{ic}: \mathbb{R}^{d \times|V|} \to \mathbb{R}$. 
    
    In the following, we will use $f = F(\cdot, \mathcal{D} \in \mathbb{D})$ to refer to the \textit{partial application} of an objective function where the corpus has been fixed. This partial application of $F$ yields a function $f: \mathcal{X} \to \mathbb{R}$ that calculates the objective value for a certain vertex embedding; different corpora now correspond to different $f$ for the same objective function $F$. 
    
    The second stage obtains the vertex embeddings by fixing the corpus $\mathcal{D}$ generated in the first stage from Algorithm~\ref{algo:corpusgeneration} in the objective function $F$ to create a partial application $f: \mathcal{X} \to \mathbb{R}$ which then is optimised with respect to the vertex embeddings by an optimisation procedure $A$. To keep our discussion as general as possible, we view the optimisation procedure as a deterministic function $A: f \mapsto \mathcal{X}$ which maps an objective function (with the corpus fixed) onto the space of vertex embeddings (the remaining argument of $f$); stochastic components can be incorporated by fixing the random seed of a pseudo-random number generator. 

    
        
        %
         \begin{algorithm}[t!]
        %
           \caption{Generating Corpus $\mathcal{D}$ on graph $G=(V, E)$}
             \label{algo:corpusgeneration}
            %
            \begin{algorithmic}[1]
                %
                %\INPUT Graph $G=(V, E)$; Transition Matrix $P$; $N, L, T\in \mathbb{N}_{>0}$; $f_{V_0}$
                %
                \STATE $m \gets \mathbf{0}_{|V|\times |V|}$
                \FOR{$n \gets 1 \textnormal{ to } N$}
                    \STATE $v_0^n \gets V_0 \sim f_{V_0}$
                    \STATE $(v_0^n, v_1^n, \dots, v_{L-1}^n) \gets \textsc{Markov}(v_0, P, L)$
                    \FOR{$j \gets 0 \textnormal{ to } L-T-1$} \label{line:secondloop}
                        \FOR{$r \gets 1 \textnormal{ to } T$}
                            \STATE $m(v_j^n, v_{j+r}^n) \gets m(v_j^n, v_{j+r}^n) + 1$
                            \STATE $m(v_{j+r}^n, v_{j}^n) \gets m(v_{j+r}^n, v_{j}^n) + 1$
                        \ENDFOR
                    \ENDFOR
                \ENDFOR
                \RETURN $\mathcal{D} = (V\times V, m)$
            \end{algorithmic}
            %\caption{Generating Corpus $\mathcal{D}$}
             %\label{algo:corpusgeneration}
        \end{algorithm}


==> LaTeX Source/sections/introduction.tex <==


\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
\IEEEPARstart{G}{raphs} naturally represent data arising in several real-world scenarios; important examples include social networks, medical records, protein networks and the web. In many tasks, using graph embeddings that meaningfully encode relevant information about the graph structure has enabled outstanding performance on downstream tasks, for example in node classification~\cite{neville2000iterative}, link prediction~\cite{liben2007link}, anomaly detection~\cite{akoglu2015graph}, and node clustering~\cite{nie2017unsupervised,aviles2019labelled}.


 
This has motivated the development of several techniques which generate embeddings by digesting the graph in different ways. One set of techniques is based on matrix factorisation, e.g.~\cite{balasubramanian2002isomap, anderson1985eigenvalues, roweis2000nonlinear, ou2016asymmetric,pang2017flexible}, in which the connections between nodes (graph properties) are represented in matrix form to obtain the embeddings. Other bodies of research have explored approaches including generative models ~\cite{le2014probabilistic,alharbi2016learning, xiao2017ssp} and hybrid (i.e. a combination of) techniques ~\cite{wei2017cross,guo2015semantically,mousavi2017hierarchical}, to name a few. 

\begin{figure}[t!]  %% teaser figure for the paper
	\begin{centering}
		\includegraphics[width=1\linewidth]{Figs/teaserV5.pdf}
		\par\end{centering}
	\caption{ Input-output of a random walk based vertex embeddings technique from one of our experiments. (a) Input graph from the Wiki dataset~\cite{yang2015network}. (b) Learned latent vertex representation generated by DeepWalk~\cite{perozzi2014deepwalk}. Colors indicate ground-truth classes in the dataset, and the high-dimensional embeddings have been visualised using t-SNE \cite{tsne}.} \label{fig:teaserIntroduction}
\end{figure}

Of particular interest for this paper are random-walk-based techniques, e.g.~\cite{perozzi2014deepwalk,grover2016node2vec,yang2016revisiting,cao2016dngr}, who have become popular due to their good performance. The core idea is to create a \textit{context} for each vertex by generating sequences of vertices using random walks on the graph before generating vertex embeddings from these contexts. Motivated by the success of neural language models, starting with the seminal DeepWalk~\cite{perozzi2014deepwalk} and followed by others including node2vec~\cite{grover2016node2vec} and DNGR~\cite{cao2016dngr}, a variety of algorithms view individual random walks as \say{sentences} consisting of individual \say{words} (individual vertices); a collection of random walks then corresponds to a \say{text corpus}. A corpus of random walks derived from a graph during a first stage can then be analysed in a second stage using language models such as SkipGram~\cite{mikolov2013skipgram}, which creates word (vertex) embeddings that allow one to predict a word's context from its embedding. This process is illustrated in \cref{fig:teaserIntroduction} using one of our experiments, where the graph input and the latent vertex representation are displayed.

%Formally, the aim in is to find an embedding (representation) for the graph $G=(V, E)$ with $V$ the vertex set of the graph and $E \subseteq V\times V$ by associating to each vertex $v\in V$ a point $z_v\in \mathbb{R}^d$, for a fixed embedding dimension $d$ much smaller than the size of the data set. Such representations leverage the graph structure to encode the relevant information into a more digestible format. This process is illustrated in Figure \ref{fig:teaserIntroduction} using one of our experiments, where the graph input and the latent representation are displayed.

%\textcolor{blue}{-}to be added deep learning random walks

%\Angie{Comment: this part should be very strong -- majority of the reviewers check the contributions and then the main results. Please feel free to add/improve any point}

%to be updated
\textbf{Contributions.} Despite their wide-spread usage, not much effort has been spent on developing a firm theoretical understanding of these algorithms. In particular, the study of the convergence of random-walk based algorithms is relatively new and incomplete.
While there are several works that slightly vary the graph sampling procedure in the first stage, e.g. \cite{grover2016node2vec} and \cite{perozzi2017don}, in this paper we mainly consider algorithms that share the sampling strategy of DeepWalk~\cite{perozzi2014deepwalk} due to this strategy's practical advantages (requiring, for example, fewer hyperparameters than node2vec~\cite{grover2016node2vec}) and because it continues to be the backbone for many new  techniques and applications, e.g.~\cite{tu2016max,qiu2018unifying,chen2019deepwalk,chen2020prediction}. 
Our contributions are:
\begin{itemize}
   \item  After formally describing DeepWalk-related techniques (\Cref{sec:formaldeepwalkdescr}), we provide a theoretical analysis for random-walk based embedding algorithms. (\Cref{sec:convergence})
   \begin{itemize}
     \item  In \cref{subsec:convrandomwalks}, we formalise the random-walk sampling strategy used by DeepWalk~\cite{perozzi2014deepwalk} in its first stage and derive the asymptotic limit of the corpora generated. We show that as the number of random walks $N$ goes to $\infty$ this convergence is almost sure both in the single limit $N \to \infty$ and the double limit $N, L \to \infty$ where $L$ is the length of each random walk. (\Cref{thm:relpairoccurrence}, \Cref{cor:longerrandomwalks})
     
     \item In \cref{subsec:convrate}, we derive concentration bounds that quantify the convergence rate of the corpora in both these cases. (\Cref{thm:Nconvspeed}, \Cref{thm:jointconvrate})
     
     \item We apply the results of this analysis to derive a heuristic that gives optimal values for the hyperparameters $N$ and $L$ for a fixed computational cost. (\Cref{cor:heuristic})
   \end{itemize}
   
   \item We validate our theoretical results %and illustrate the advantages of the optimal choice of hyperparameters 
   through a set of experiments using medium-sized and large real-world graphs consisting of thousands to millions vertices / edges. (\Cref{sec:experiments})
 \end{itemize}


%% ---

%   Many real-world datasets of interest are naturally represented as graphs, for instance, social networks, the internet as a whole, or financial transactions.
%     A popular pre-processing step, before tasks such as classification, is to find a vertex representation of the graph in a much lower dimensional space; that is, we wish to associate to each vertex $v\in V$ a point $z_v\in \mathbb{R}^d$, for a fixed $d$ much smaller than the size of the data set. Such representations leverage the graph structure and should encode the important information in the graph in a simple way. Consequently, many algorithms have been developed to obtain these representations \cite{zhang2018networkembeddingsurvey}; the object of our interest is the seminal DeepWalk algorithm \cite{perozzi2014deepwalk}, which was the first of a class of random-walk-based algorithms including node2vec \cite{grover2016node2vec} and DNGR \cite{cao2016dngr}. The general idea is to generate vertex sequences using random walks and then learn vertex embedings using techniques originally developed for Natural Language Processing, treating the random walks as `sentences' and the vertices as `words'. DeepWalk itself uses the SkipGram algorithm \cite{mikolov2013skipgram} to create vertex embedings from a corpus of  `sentences' obtained from random walks.

%     Despite their wide-spread usage, not much effort has been spent on developing a firm theoretical understanding of these algorithms. In particular, the convergence of random-walk based algorithms for vertex embedding has not been deeply investigated. The goal of this present work is to investigate the limiting behaviour, and to quantify, as far as possible, the rate of convergence.
    
%   The paper is structured as follows. In Section \ref{sec_convergence} we formally introduce the DeepWalk algorithm (\ref{subsec_formaldeepwalkintro}) in order to fix notation and terminology. , followed by the derivation of convergence guarantees for DeepWalk (\ref{subsec_convvertexreps} and \ref{subsec_convrandomwalks}) and a discussion of the rate of this convergence (\ref{subsec_convrate}). The section will close with a look at the behaviour of DeepWalk when applied to dynamic graphs (\ref{subsec_deepwalkdynamicgraphs}).

%     The results from \ref{sec_convergence} are further discussed in \ref{sec_discussion}. We give possible interpretations of the learned vertex embeddings (\ref{subsec_interpretvertexreps}) and briefly discuss the relevance of the previous results to real-world applications of DeepWalk (\ref{subsec_relevancepractice}). 




==> LaTeX Source/sections/relatedwork.tex <==
\section{Related Work} \label{sec:relatedwork}
%The body of literature has reported several techniques for graph embeddings.
%In particular, and motivated by their performance, deep learning techniques have become a great focus of attention, in which techniques roughly be categorised on whether random walks are applied for sampling the graph paths.   In this work, we are instead interested in random walk based techniques, which have demonstrated high performance. In this section, we review the existing techniques in turn.

This paper is interested in random-walk-based techniques for vertex embeddings, which have demonstrated outstanding performance. We first briefly review existing such techniques.

\smallskip
\textbf{Random-Walk Based Vertex Embeddings.} The seminal work of Perozzi et al.~\cite{perozzi2014deepwalk} introduced the DeepWalk technique, which learns embeddings in two stages. In the first stage, a given graph is sampled using random walks, followed by an application of the SkipGram model to then generate vertex embeddings that allow one to predict the vertices that appear within a window around the vertex in the random walks. The promising performance of the DeepWalk motivated the developments of subsequent techniques that follow the principles of the DeepWalk.
%with some variants in the sampling strategies or  (e.g.,~\cite{grover2016node2vec,yang2016revisiting}) or proximity constraints (e.g.,~\cite{li2016discriminative,yang2015multi}).}

%
Grover et al.~\cite{grover2016node2vec} introduce an additional parameter to control the random walks by allowing the user to interpolate between breadth-first and depth-first graph searches. Another modification of the first stage called Walklets was introduced in \cite{perozzi2017don}, where authors skipped over steps in each random walk. The HARP model introduced in \cite{chen2018harp} improves the initialisation of the SkipGram stage. Slightly improved performance of these models compared to DeepWalk however comes at the cost of increased computational costs.
Another set of techniques modified DeepWalk by introducing different sampling techniques for the random walks (e.g.~\cite{yang2016revisiting,pimentel2017unsupervised}), and enforcing preservation of some graph properties (e.g.~\cite{yang2015multi,pan2016tri,li2016discriminative}). Other variants of the such family of techniques are the works of~\cite{tang2015line, cao2015grarep, ou2016asymmetric, cao2016dngr}.
There exist also techniques that aim to create similar network embeddings without (explicitly) sampling any random walks, for example \cite{chen2019fastrp}. 


While DeepWalk and its variants have been widely explored in the literature from a practical point of view, the analysis of the theoretical properties of such techniques is still relatively new. There are only few works that discussed the theoretical properties of this family of techniques. In the following, we discuss them and note the differences with the present work.

\smallskip
\textbf{Theoretical Analyses of DeepWalk \& Comparison to Our Work.} The first theoretical analysis of random-walk based vertex embedding techniques is due to Qiu et al.~\cite{qiu2018unifying}, who demonstrated a relationship between DeepWalk and a particular matrix factorisation problem. In the notation of \cref{sec:formaldeepwalkdescr}, that work identifies the limiting behaviour as the length of the walk $L\to\infty$, but does not prove a quantitative rate, and keeps the number of trials $N$ fixed rather than identifying the convergence as $N\to \infty$ or the convergence of the joint limit as done here. The behaviour of DeepWalk in the limit of many shorter (instead of fewer long) random walks as investigated in our work arguably has greater practical relevance as it allows for much easier parallelisation of the algorithm. Additionally, the proof in \cite{qiu2018unifying} only applies to undirected, non-bipartite graphs whereas our \Cref{thm:relpairoccurrence} and Corollaries \ref{cor:longerrandomwalks} and \ref{cor:effectstartingdistr} apply to directed and undirected graphs, both periodic and aperiodic.

More recently, another work \cite{qiu2020matrix} proved a concentration bound in terms of $L$ for arbitrary $N$ for the convergence of a corpus of random walks generated from an aperiodic graph. In contrast, we derive concentration bounds in terms of $N$ for arbitrary $L$ (\Cref{thm:Nconvspeed}) and in terms of $N$ and $L$ for the joint limit (\Cref{thm:jointconvrate}) for both periodic and aperiodic graphs. Furthermore, our bounds do not depend on the size of the graph, a factor that while of constant order can be very significant in real-world graphs with vertices and edges potentially numbering in the millions (cf. \cref{table:datasets}). In this paper, we also consider the assumptions necessary for convergence of the co-occurrence matrix to imply convergence of the extracted vertex representations (\Cref{thm:convvertexreps}), a question that \cite{qiu2020matrix} does not address.

Most recently, \cite{zhang2021consistency} considers random graphs, in either the sparse or dense regimes, in the asymptotic where the size $|V|$ and the number of sampled paths $N\to \infty$ on a fixed time interval. While also investigating the theoretical properties of random-walk based graph embedding algorithms, the setting that they consider is different to the one considered in this paper or, in fact, in~\cite{qiu2020matrix}.

Moreover and in contrast to the works above, we illustrate the practical relevance of our analysis in \Cref{cor:heuristic} by combining our results to derive a rule for the optimal choice of the hyperparameters $N$ and $L$. Qiu et al. \cite{qiu2020matrix} also derive a heuristic for choosing $L$, but they assume implicitly that $N=1$, which as our experiments in \cref{sec:experiments} show yields worse task-performance than our heuristic.
